Learning in Proportional Allocation Auctions Games

The Kelly or proportional allocation mechanism is a simple and efficient auction-based scheme that distributes an infinitely divisible resource proportionally to the agents bids. When agents are aware of the allocation rule, their interactions form a game extensively studied in the literature. This paper examines the less explored repeated Kelly game, focusing mainly on utilities that are logarithmic in the allocated resource fraction. We first derive this logarithmic form from fairness-throughput trade-offs in wireless network slicing, and then prove that the induced stage game admits a unique Nash equilibrium NE. For the repeated play, we prove convergence to this NE under three behavioral models: (i) all agents use Online Gradient Descent (OGD), (ii) all agents use Dual Averaging with a quadratic regularizer (DAQ) (a variant of the Follow-the-Regularized leader algorithm), and (iii) all agents play myopic best responses (BR). Our convergence results hold even when agents use personalized learning rates in OGD and DAQ (e.g., tuned to optimize individual regret bounds), and they extend to a broader class of utilities that meet a certain sufficient condition. Finally, we complement our theoretical results with extensive simulations of the repeated Kelly game under several behavioral models, comparing them in terms of convergence speed to the NE, and per-agent time-average utility. The results suggest that BR achieves the fastest convergence and the highest time-average utility, and that convergence to the stage-game NE may fail under heterogeneous update rules.

==> journal/draft_experiments.tex <==



\subsection{Previous version}

% \begin{table}[t]
% \centering
% \caption{Performance metrics.}
% \label{tab:metrics}
% \begin{tabular}{lll}
% \toprule
% Metric & Symbol & Interpretation \\
% \midrule
% Normalized payoff & $\overline{\varphi_i}$ & Individual utility (normalized) \\
% Efficiency loss & $\rho$ & Welfare gap to optimum \\
% $\epsilon$-Nash proximity & $\epsilon(\bm z)$ & Incentive to deviate \\
% Fixed-point residual & $r_t$ & Action-space consistency \\
% \bottomrule
% \end{tabular}
% \end{table}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}
\begin{minipage}{0.48\textwidth}%[!t]
    \centering

    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=\textwidth]{img/Hybrid/Payoff/DAQ_F_legend.pdf}\\[0.5ex]

    %--- Ligne de sous-figures (4 colonnes) ---
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Payoff/1_SBRD_9_DAQ_F_Payoff_alpha1_gamma0.0_n_10_plot.pdf}

            % Rectangle de zoom
            \put(67,53){\color{black}\linethickness{0.7pt}\framebox(30,10){}}

            % Image zoomée (UTILISER \linewidth, PAS \textwidth)
            \put(31,14){
                \includegraphics[width=0.4\linewidth]
                {img/Hybrid/Payoff/Zoom_1_SBRD_9_DAQ_F_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
            }

            % Flèche vers le zoom
            \linethickness{1pt}
            \put(50,32){\vector(1,1){18}}
        \end{overpic}
        \caption{$\alpha_{\texttt{BR}} = 10\%$}
        \label{fig:1_SBRD_9_DAQ_F_Payoff}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{img/Hybrid/Payoff/SBRD_DAQ_F_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
            
        \caption{\scriptsize{$\alpha_{\texttt{BR}}  [10\%,\;80\%]$}}
         \label{fig:SBRD_DAQ_F_Payoff}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Payoff/9_SBRD_1_DAQ_F_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{\texttt{BR}} = 90\%$}
         \label{fig:9_SBRD_1_DAQ_F_Payoff}
    \end{subfigure}

    \caption{heterogeneous dynamics: \textbf{Average(avg.) and instantaneous(inst.) payoff,} \texttt{BR} vs \texttt{DAQ}$_F$.}
    \label{fig:Hybrid_SBRD_DAQ_F_utility_compare0.0_n_10}
\end{minipage}
%    \centering
\begin{minipage}{0.48\textwidth}
    \centering

    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=\textwidth]{img/Hybrid/Payoff/OGD_V_legend.pdf}\\[0.5ex]

    %--- Ligne de sous-figures (4 colonnes) ---
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Payoff/1_SBRD_9_OGD_V_Payoff_alpha1_gamma0.0_n_10_plot.pdf}

            % Rectangle de zoom
            \put(67,53){\color{black}\linethickness{0.7pt}\framebox(30,10){}}

            % Image zoomée (proportionnelle à la sous-figure)
            \put(31,14){
                \includegraphics[width=0.4\linewidth]
                {img/Hybrid/Payoff/Zoom_1_SBRD_9_OGD_V_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
            }

            % Flèche vers le zoom
            \linethickness{1pt}
            \put(50,32){\vector(1,1){18}}
        \end{overpic}
        \caption{$\alpha_{\texttt{BR}} = 10\%$}
        \label{fig:1_SBRD_9_OGD_V_Payoff}
    \end{subfigure}
        \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{img/Hybrid/Payoff/SBRD_OGD_V_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
        \caption{\scriptsize{$\alpha_{\texttt{BR}} [10\%,\;80\%]$}}
        \label{fig:SBRD_OGD_V_Payoff}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Payoff/9_SBRD_1_OGD_V_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{\texttt{BR}} = 90\%$}
        \label{fig:9_SBRD_5_OGD_V_Payoff}
    \end{subfigure}

    \caption{heterogeneous dynamics: \textbf{Average(avg.) and instantaneous(inst.) payoff,} \texttt{BR} vs \texttt{OGD}$_V$.}
    \label{fig:Hybrid_SBRD_OGD_V_utility_compare0.0_n_10}
\end{minipage}
\end{figure*}


\begin{figure*}[t]
\begin{minipage}{0.48\textwidth}%[!t]
    \centering

    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=\textwidth]{img/Hybrid/Payoff/RRM_V_legend.pdf}\\[0.5ex]

    %--- Ligne de sous-figures (4 colonnes) ---
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Payoff/1_SBRD_9_RRM_V_Payoff_alpha1_gamma0.0_n_10_plot.pdf}

        \end{overpic}
        \caption{$\alpha_{\texttt{BR}} = 10\%$}
        \label{fig:1_SBRD_9_RRM_V_Payoff}
    \end{subfigure}
       \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/Hybrid/Payoff/SBRD_RRM_V_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
        \caption{\scriptsize{$\alpha_{\texttt{BR}} [10\%,\;80\%]$}}
        \label{fig:SBRD_RRM_V_Payoff}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]
            {img/Hybrid/Payoff/9_SBRD_1_RRM_V_Payoff_alpha1_gamma0.0_n_10_plot.pdf}

        \caption{$\alpha_{\texttt{BR}} = 90\%$}
        \label{fig:9_SBRD_1_RRM_V_Payoff}
    \end{subfigure}

    \caption{heterogeneous dynamics: \textbf{Average(avg.) and instantaneous(inst.) payoff}, \texttt{BR} vs \texttt{RRM}$_V$.}
    \label{fig:Hybrid_SBRD_RRM_V_utility_compare0.0_n_10}
\end{minipage}
\begin{minipage}{0.48\textwidth}%[!t]
    \centering

    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=\textwidth]{img/Hybrid/Payoff/OGD_V_vs_DAQ_F_legend.pdf}\\[0.5ex]

    %--- Ligne de sous-figures (4 colonnes) ---
            \begin{subfigure}[b]{0.32\textwidth}
        \centering
\includegraphics[width=\linewidth]{img/Hybrid/Payoff/OGD_V_DAQ_F_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
        \caption{\scriptsize{$\alpha_{\text{OGD}_V} [20\%,\;80\%] $}}
        \label{fig:DAQ_F_OGD_V_Payoff}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Payoff/1_OGD_V_9_DAQ_F_Payoff_alpha1_gamma0.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{\text{OGD}_V} = 10\%$}
        \label{fig:1_OGD_V_9_DAQ_F_Payoff}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Payoff/1_DAQ_F_9_OGD_V_Payoff_alpha1_gamma0.0_n_10_plot.pdf}

        \end{overpic}
        \caption{$\alpha_{\text{OGD}_V} = 90\%$}
        \label{fig:1_DAQ_F_9_OGD_V_Payoff}
    \end{subfigure}
    \caption{heterogeneous dynamics: \textbf{Average(avg.) and instantaneous(inst.) payoff,} \texttt{OGD}$_V$ vs \texttt{DAQ}$_F$.}
    \label{fig:Hybrid_OGD_V_DAQ_F_utility_compare0.0_n_10}
\end{minipage}
\end{figure*}


\begin{itemize}
    \item \textbf{$\epsilon$-Nash proximity ($\epsilon(\bm z(t))$)} (maximum unilateral utility gain).
    
    \begin{equation}\label{eq:metric_epsilon_error}
        \epsilon(\bm z(t))= \max_i\left[
        \overline{\varphi_i}\left(\BR_i(\bm z_{-i}(t)),\bm z_{-i}(t)\right)-
        \overline{\varphi_i}\left(\bm z(t)\right)
        \right].
    \end{equation}
    
    \item \textbf{Fixed-point residual} (distance to the best-response fixed point).
    
    \begin{equation}\label{eq:metric_residual}
    r_t=\|\BR(\bm z(t))-\bm z(t)\|_2 .
    \end{equation}
    \textcolor{blue}{ Interesting ~\cite[Thm.~2]{hazan2007computational}, I will change the average payoff to the payoff of average actions} \YBnote{I think the time-average payoff is more important from an online optimization perspective. }
    \item \textbf{Normalized payoff} (instantaneous and time-averaged utility).

\begin{equation}\label{eq:metric_utility}
\overline{\varphi_i}(\bm z)=
\frac{\varphi_i(\bm z)-\varphi_i^{\min}}{\varphi_i^{\max}-\varphi_i^{\min}},
\qquad
\frac{1}{T}\sum_{t=1}^T \overline{\varphi_i}(\bm z(t)),
\end{equation}
where $\varphi_i^{\min}=\min\{\varphi_i(c_i,\bm c_{-i}),\varphi_i(\epsilon,\bm c_{-i})\}$ and
$\varphi_i^{\max}=\varphi_i(\BR_i(\bm\epsilon_{-i}),\bm\epsilon_{-i})$. In the symmetric-agents case ($a_i=a$), the symmetric NE $z^\star$ satisfies $n(z^\star)^2-z^\star(a(n-1)-\delta)-a\delta=0,$ and serves as a benchmark.
%In the homogeneous case, the symmetric NE payoff serves as a benchmark.
\item \textbf{Relative efficiency loss ($\rho(\bm{z}(t))$)}: let $\mathrm{SW}(\bm z)\triangleq \sum_{i\in\mathcal I}V_i(x_i(\bm z))$ denote social welfare and let $\bm z^{opt}$ be a welfare-optimal bid profile. We report
\begin{equation}\label{eq:metric_loss}
\rho(\bm z (t))=
\left|
\frac{\mathrm{SW}(\bm z(t))-\mathrm{SW}(\bm z^{opt})}{\mathrm{SW}(\bm z^{opt})}
\right|.
\end{equation}

\end{itemize}

We present numerical experiments that (i) validate the theoretical guarantees established for the repeated Kelly game and (ii) quantify the impact of algorithmic heterogeneity.

Our simulations include both \textbf{homogeneous dynamics} settings, where all agents follow the same update rule, and \textbf{heterogeneous dynamics} settings, where a fraction $\alpha_{\mathcal{A}_1}=k/n$ of agents use algorithm $\mathcal{A}_1$ while the remaining agents use $\mathcal{A}_2$.


% \YBnote{\begin{itemize}
%     \item I propose to focus first on the convergence speed, then the payoff comparison across players. Maybe at the end, we can add results for the efficiency loss. For similar reasons that we mentioned in the conference paper. 
    
% \end{itemize}}


%\subsection{Experimental Configurations}

% We consider two configurations:
% \begin{itemize}
%     \item \textbf{homogeneous dynamics:} all agents use the same update rule, isolating the intrinsic behavior of each algorithm.
%     \item \textbf{heterogeneous dynamics:} a fraction $\alpha_{A_1}=k/n$ of agents use algorithm $A_1$, while the remaining agents use $A_2$, capturing algorithmic heterogeneity.
    
% \end{itemize}


% ----------------------------------------------------------
\subsection{Homogeneous dynamics}
% ----------------------------------------------------------
\href{https://app-kellymechanism-simulation.streamlit.app/}{\textcolor{red}{Simulation (to be DELETE)}}

% ----------------------------------------------------------
We begin with the \textbf{homogeneous dynamics} configuration.








%%%%%%%%%%%%%%%%%%%%%% Tables %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
% \begin{minipage}{0.48\textwidth}
% \centering
% \captionof{table}{Homogeneous dynamics: \textbf{Convergence iterations} in terms of 
% \textbf{fixed-point residual} $r_t$ under varying $\gamma$ and $n$. \YBnote{add the target precision required here.}}
% \label{tab:convergence_residual}
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{$\gamma$} & \textbf{$n$} 
% & \textbf{\texttt{BR}} 
% & \textbf{\texttt{OGD}$_V$} 
% & \textbf{\texttt{OGD}$_F$} 
% & \textbf{\texttt{DAQ}$_F$} 
% & \textbf{\texttt{DAQ}$_V$} 
% & \textbf{\texttt{RRM}$_V$} \\
% \hline
% \multirow{3}{*}{\textbf{0}}
% & 2   & 15 & 37 & 122 & 195 & $(r_T=3.7{\times}10^{-2})$ & 1682  \\
% & 10  & 7  & 19 & 240 & 311 & $(r_T=1.05)$              & 2291 \\
% & 20  & 6  & 20 & 252 & 330 & $(r_T=1.73)$              & 2361 \\
% \hline

% \multirow{3}{*}{\textbf{5}}
% & 2   & 15 & 39 & 127 & 184 & $(r_T=1.0{\times}10^{-1})$ & 504  \\
% & 10  & 7  & 16 & 206 & 274 & $(r_T=6.8{\times}10^{-1})$ & 2182 \\
% & 20  & 6  & 501 & 221 & 289 & $(r_T=7.5{\times}10^{-1})$ & 2220 \\
% \hline

% \multirow{3}{*}{\textbf{10}}
% & 2  & 15 & 41  & 117 & 184 & $(r_T=9.7{\times}10^{-2})$ & 498   \\
% & 10 & 8  & 160 & 185 & 253 & $(r_T=4.5{\times}10^{-1})$ & 1604 \\
% & 20 & 8  & 160 & 194 & 259 & $(r_T=4.5{\times}10^{-1})$ & 2062 \\
% \hline
% \end{tabular}
% \end{minipage}
% \hfill 
\begin{minipage}{0.48\textwidth}
\centering
\captionof{table}{Homogeneous dynamics: \textbf{Convergence iterations} in terms of 
\textbf{$\bm{\epsilon}$-Nash proximity} under varying $\gamma$ and $n$.}
\label{tab:convergence}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{$\gamma$} & \textbf{$n$} 
& \textbf{\texttt{BR}} 
& \textbf{\texttt{OGD}$_V$} 
& \textbf{\texttt{OGD}$_F$} 
& \textbf{\texttt{DAQ}$_F$} 
& \textbf{\texttt{DAQ}$_V$} 
& \textbf{\texttt{RRM}$_V$} \\
\hline
\multirow{3}{*}{\textbf{0}}
& 2   & 9 & 30 & 79  & 152 & $(\epsilon_T=4.6{\times}10^{-5})$ & 1652  \\
& 10  & 4 & 10 & 149 & 219 & $(\epsilon_T=2.0{\times}10^{-4})$ & 2212 \\
& 20  & 3 & 10 & 149 & 228 & $(\epsilon_T=2.0{\times}10^{-4})$ & 2271 \\
\hline

\multirow{3}{*}{\textbf{5}}
& 2   & 9 & 33 & 86  & 142 & $(\epsilon_T=1.3{\times}10^{-4})$ & 489  \\
& 10  & 4 & 11 & 127 & 192 & $(\epsilon_T=3.5{\times}10^{-4})$ & 2111 \\
& 20  & 4 & 215 & 135 & 195 & $(\epsilon_T=2.8{\times}10^{-4})$ & 2139 \\
\hline

\multirow{3}{*}{\textbf{10}}
& 2  & 9 & 34  & 78  & 145 & $(\epsilon_T=1.3{\times}10^{-4})$ & 484   \\
& 10 & 5 & 135 & 113 & 179 & $(\epsilon_T=2.6{\times}10^{-4})$ & 1554 \\
& 20 & 4 & 134 & 119 & 182 & $(\epsilon_T=2.3{\times}10^{-4})$ & 2000 \\
\hline
\end{tabular}
\end{minipage}


\end{table}


\paragraph{\textbf{Convergence speed.}}
Convergence is evaluated via the maximum unilateral utility gain, $\epsilon(\bm z(t))$, and the distance to the \texttt{BR} fixed point, $\|\BR(\bm z(t))-\bm z(t)\|_2$, using a tolerance of $10^{-5}$.


Figure~\ref{fig:epsilon_summary} shows that, in the homogeneous dynamics, all algorithms, excepts \texttt{DAQ}$_V$  reach the prescribed target precision. In the symmetric-agent setting (Fig.~\ref{fig:epsilon_error_alpha1_gamma0}), convergence is fastest under \texttt{BR}, followed by \texttt{OGD}$_V$, \texttt{OGD}$_F$, and \texttt{DAQ}$_F$. In contrast, \texttt{RRM}$_V$ requires significantly more iterations, which is consistent with the fact that for \texttt{RRM}$_V$, we don't have  no-regret guarantees and may allow large $\epsilon$-Nash proximity values during the transient phase before converging. Finally, \texttt{DAQ}$_V$ is by far the slowest, a behavior that is not surprising since, when the horizon $T$ is known, tighter regret guarantees are obtained with fixed step sizes, as in \texttt{DAQ}$_F$ \cite[Sec.~3.2]{McMahan_FTRL_JMLR_17}.
For all learning-based methods, when it converges, convergence time increases only marginally with the number of agents. By contrast, \texttt{BR} converges faster as the population grows, while convergence remains approximately insensitive to agent heterogeneity across all algorithms (Table~\ref{tab:convergence}).




Action-space convergence, a stricter notion of equilibrium attainment, is measured by the fixed-point residual in Figure~\ref{fig:Homogeneous_speed_subfigs}, confirming the same algorithmic ranking, while typically occurring more slowly than convergence in utility space, which is more pronounced in \texttt{DAQ}$_V$'s curve. This behavior is expected, as convergence in strategies implies convergence in payoffs. Table~\ref{tab:convergence_residual} summarizes these results and shows that \texttt{DAQ}$_V$ may fail to converge in strategy under several configurations ($T=3000$).








\paragraph{\textbf{Payoff.}}
Figure~\ref{fig:non-hybrid_avg_payoff} reports instantaneous and time-averaged payoffs in the symmetric-agent setting. 
Across algorithms, payoffs concentrate around the Nash benchmark, indicating stable equilibrium behavior in utility space. 
While \texttt{RRM}$_V$ exhibits slower adjustment in the time-average, its instantaneous payoff eventually aligns with the equilibrium level. 
Overall, the results are consistent with the theoretical prediction that no-regret learning ensures convergence of time-averaged utilities to the stage-game Nash equilibrium payoff~\cite[Thm.~2]{hazan2007computational}.





%We now turn to the objective function that each player seeks to maximize. This complements Fig.~\ref{fig:Hybrid_Dis2SW}, which focused on social welfare, by examining instead the evolution of individual payoffs under different learning rules. In the following experiments, we will consider only homogeneous players for better visualization. 

%Fig.~\ref{fig:utility_compare0.0_n_10} illustrates how a player's utility depends on the fraction 
%of agents using SBRD ($\alpha_{\texttt{BR}}$.
%The player can choose either SBRD or DAE. When using SBRD, the player's utility increases as 
%more agents adopt SBRD, and it consistently outperforms DAE. For DAE, utility also improves 
%with the share of SBRD users, but the gap between the two grows as the fraction of SBRD players increases. Once SBRD dominates the population, its advantage over DAE becomes even more pronounced. Building on the results of Fig.~\ref{fig:Hybrid_Dis2SW}, where SBRD users strongly dominate, this configuration leads to a lower overall SW. The reason is that SBRD users achieve higher individual utilities, while the others obtain significantly lower payoffs.











%\caption{homogeneous dynamics: \textbf{$\bm{\epsilon}$-Nash Proximity}   across algorithms for varying heterogeneity levels $\gamma$.}
    %\label{fig:epsilon_error_non_hybrid}


\paragraph{ \textbf{Relative Efficiency Loss ($\rho$)}} 
The Kelly mechanism guarantees that at Nash equilibrium (NE),
\(\mathrm{SW}(\mathbf{z}^{NE}) \ge \tfrac{3}{4}\mathrm{SW}(\mathbf{z}^{opt})\)~\cite{johari_thesis2004},  
implying a worst-case efficiency loss of \(\rho(\mathbf{z}^{NE}) \le 25\%\).  
Figure~\ref{fig:SBRD_REL_alpha1_gamma0_n_10} confirms that in the homogeneous dynamics, all algorithms achieve
\(\rho(\mathbf{z}(t)) \ll 25\%\), thus operating near the optimal social welfare.  
Although \(\rho\) slightly increases for heterogeneous environments (\(\gamma>0\)), figs.~\ref{fig:SBRD_REL_alpha1_gamma5_n_10}--\ref{fig:SBRD_REL_alpha1_gamma10_n_10}, the ranking among methods remains consistent across all configurations.







%The results indicate that SBRD is robust with respect to parameter variations and consistently achieves fast convergence. Interestingly, increasing the number of players $n$ appears to further accelerate the convergence of SBRD, where no-regrets require more iterations.





\subsection{Heterogeneous dynamics}
\begin{itemize}
    \item average payoff marker fixed T=3000
    \item Fixed bids $\alpha_{\texttt{BR}}$, 3 values; the extrema include
\end{itemize}

We now examine Heterogeneous dynamics, in the case where two algorithms coexist.  
Players adopt either \texttt{BR} or one of \texttt{DAQ}$_F$ or  \texttt{OGD}$_V$. Or by mixing two no regret  
We first vary the fraction of \texttt{BR} users, denoted $\alpha_{\texttt{BR}} = k/n$,  
and then study the case where the proportion of \texttt{OGD}$_V$ users, $\alpha_{\texttt{OGD}_V} = k/n$, is varied instead. To avoid favoring a specific rule, all hybrid experiments start from the same initial bid profile.


\paragraph{\textbf{Payoff}}  
%%%%%%%%%Payoff%%%%%%%%%%%%%%%%%




We begin the hybrid analysis by examining instantaneous and time-averaged payoffs.  
Figure~\ref{fig:Hybrid_SBRD_DAQ_F_utility_compare0.0_n_10} illustrates interactions between \texttt{BR} and \texttt{DAQ}$_F$ players.  
For a small fraction of \texttt{BR} users ($\alpha_{\texttt{BR}}=10\%$, Fig.~\ref{fig:1_SBRD_9_DAQ_F_Payoff}), both payoffs converge to values close to the Nash equilibrium, with \texttt{BR} consistently achieving higher utility.  
As $\alpha_{\texttt{BR}}$ increases (Fig.~\ref{fig:SBRD_DAQ_F_Payoff}), the payoff gap widens in favor of \texttt{BR}: utilities initially increase for all players and exceed the NE level, but beyond $\alpha_{\texttt{BR}}=50\%$ the utility of \texttt{DAQ}$_F$ players decreases, falling below the NE for $\alpha_{\texttt{BR}}\ge80\%$.

At $\alpha_{\texttt{BR}}=90\%$ (Fig.~\ref{fig:9_SBRD_1_DAQ_F_Payoff}), the system enters a critical regime in which \texttt{DAQ}$_F$ players experience severe utility degradation and the instantaneous payoff exhibits persistent oscillations, preventing stabilization.  
Similar behaviors are observed when \texttt{BR} interacts with \texttt{OGD}$_V$ (Figs.~\ref{fig:1_SBRD_9_OGD_V_Payoff}--\ref{fig:9_SBRD_5_OGD_V_Payoff}), although convergence is faster than in the \texttt{DAQ}$_F$ case.  
In contrast, \texttt{BR}–\texttt{RRM}$_V$ interactions (Figs.~\ref{fig:1_SBRD_9_RRM_V_Payoff}--\ref{fig:9_SBRD_1_RRM_V_Payoff}) exhibit slower and less stable convergence, despite eventual payoff stabilization.

When two no-regret algorithms interact, as in the \texttt{DAQ}$_F$–\texttt{OGD}$_V$ case (Fig.~\ref{fig:Hybrid_OGD_V_DAQ_F_utility_compare0.0_n_10}), both payoffs display a nearly symmetric behavior around the balanced configuration $\alpha_{\texttt{OGD}_V}=50\%$.  
At extreme imbalances (e.g., $\alpha_{\texttt{OGD}_V}=10\%$ or $90\%$), the minority group suffers significant utility losses and payoff oscillations, hindering stabilization.

Overall, these experiments reveal a strong form of algorithmic externality: increasing the proportion of \texttt{BR} users benefits them both individually and collectively, while \texttt{DAQ}$_F$, \texttt{OGD}$_V$, and \texttt{RRM}$_V$ users experience reduced payoffs when outnumbered.


%For the following metrics (relative efficiency loss and convergence), we therefore restrict the analysis to cases where $\alpha_{A_1} < 80\%$, since beyond this threshold at least one algorithm may fail to stabilize.



\paragraph{\textbf{Relative Efficiency Loss ($\rho$)}}  

\begin{figure*}[!t]
\centering
    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=0.3\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]
\begin{minipage}{0.48\textwidth}
    \centering

    %--- Ligne de sous-figures (4 colonnes) ---
            \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Loss/Relative_Efficienty_Loss_alpha1_gamma0.0_player_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{SBRD}\in[10\%,\;80\%]$}
        \label{fig:Hybrid_Relative_Efficienty_Loss_alpha1_gamma0}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Loss/9_SBRD_1_Relative_Efficienty_Loss_alpha1_gamma0.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{SBRD} = 90\%$}
        \label{fig:9_SBRD_1_Relative_Efficienty_Loss_alpha1_gamma0}
    \end{subfigure}

    \caption{\texttt{BR} + $A_2$, \textbf{Relative Efficienty Loss} $(\gamma=0)$}
    \label{fig:Hybrid_Relative_Efficienty_Loss}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering

    %--- Légende globale sur toute la largeur ---
    %\includegraphics[width=\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]

    %--- Ligne de sous-figures (4 colonnes) ---

            \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/epsilon_error_alpha1_gamma0.0_player_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{SBRD}\in[10\%,\;80\%]$}
        \label{fig:Hybrid_epsilon_error_alpha1_gamma0}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/9_SBRD_1_epsilon_error_alpha1_gamma0.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{SBRD} = 90\%$}
        \label{fig:9_SBRD_1_epsilon_error_alpha1_gamma0}
    \end{subfigure}
    \caption{\texttt{BR} + $A_2$, \textbf{$\bm{\epsilon}$-Nash Proximity} $(\gamma=0)$}
    \label{fig:9_SBRD_1_Relative_Efficienty_Loss}
\end{minipage}
\end{figure*}

Figure~\ref{fig:Hybrid_Relative_Efficienty_Loss} evaluates the system efficiency in the heterogeneous dynamics by tracking the relative efficiency loss as the fraction of \texttt{BR} users ($\alpha_{\texttt{BR}}$) increases.  
Since earlier results showed that at least one group may fail to stabilize when $\alpha_{\texttt{BR}}>80\%$, and due to space constraints, we report only the final-iteration values for $\alpha_{\texttt{BR}}\le80\%$.  
Figure~\ref{fig:Hybrid_Relative_Efficienty_Loss_alpha1_gamma0} shows that, for homogeneous players, the loss increases steadily with $\alpha_{\texttt{BR}}$, indicating that more aggressive best-response dynamics worsen efficiency as \texttt{BR} becomes dominant.  
This trend persists even under heterogeneous populations (Appendix Figs.~\ref{fig_app:OGD_V_Nash_Proximity_FixPoint}).  
Nevertheless, the efficiency loss remains well below the $25\%$ worst-case bound of the Kelly mechanism~\cite{johari_thesis2004}, showing that the system retains good performance despite imbalance.  
When $\alpha_{\texttt{BR}} = 90\%$ (Fig.~\ref{fig:9_SBRD_1_Relative_Efficienty_Loss}), oscillations reappear, confirming that extreme population asymmetries can prevent the system from achieving a stable efficiency level.


\paragraph{\textbf{Convergence speed: ($\epsilon(\bm{z}(t))$)}}





\begin{figure*}[!t]
    %--- Légende globale sur toute la largeur ---
    \centering
    \includegraphics[width=0.3\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]
\begin{minipage}{0.48\textwidth}
    \centering



    %--- Ligne de sous-figures (4 colonnes) ---
            \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/Speed_alpha1_gamma0.0_player_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{SBRD}\in[10\%,\;80\%]$}
        \label{fig:Hybrid_Speed_alpha1_gamma0}
    \end{subfigure}
        %--- Ligne de sous-figures (4 colonnes) ---
            \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/9_SBRD_1_Speed_alpha1_gamma0.0_n_10_plot.pdf}

        % ---- Rectangle for zoom region ----
        % (x,y) = bottom-left corner of rectangle in percent coordinates of the image
        % (width,height) also in percent
        \put(35,10){\color{black}\linethickness{0.7pt}\framebox(60,10){}}
    
        % ---- Insert zoomed image ----
        \put(42.8,30.1){
            \includegraphics[width=0.45\textwidth]{img/Hybrid/Fix_Point_Err/Zoom_9_SBRD_1_Speed_alpha1_gamma0.0_n_10_plot.pdf}
        }
    
        % ---- Arrow connecting region to zoom ----
        \linethickness{1pt}
        \put(50,35){\vector(-1,-1){15}} % Adjust arrow slope and length if needed            
        \end{overpic}
        \caption{$\alpha_{SBRD}=90\%$}
        \label{fig:9_SBRD_1_Fix_Point_Err_alpha1_gamma0}
    \end{subfigure}
    \caption{\texttt{BR} + $A_2$, \textbf{Fixed-Point Residues} $(\gamma,\alpha_{SBRD})$}
    \label{fig:Hybrid_Speed}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering

    %--- Légende globale sur toute la largeur ---
   % \includegraphics[width=\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]


            \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/Hybrid_OGD_V_epsilon_error_alpha1_gamma0.0_n_10_plot.pdf}
        % ---- Rectangle for zoom region ----
        % (x,y) = bottom-left corner of rectangle in percent coordinates of the image
        % (width,height) also in percent
        \put(27,10){\color{black}\linethickness{0.7pt}\framebox(60,10){}}
    
        % ---- Insert zoomed image ----
        \put(35.8,25.1){
            \includegraphics[width=0.45\textwidth]{img/Hybrid/Epsilon_Error/Zoom_Hybrid_OGD_V_epsilon_error_alpha1_gamma0.0_n_10_plot.pdf}
        }
    
        % ---- Arrow connecting region to zoom ----
        \linethickness{1pt}
        \put(42,35){\vector(-1,-1){15}} % Adjust arrow slope and length if needed
        \end{overpic}
        \caption{$\alpha_{OGD_V}\in[10\%,\;90\%]$}
        \label{fig:Hybrid_OGD_V_epsilon_error_alpha1_gamma0}
    \end{subfigure}
            \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/Hybrid_OGD_V_Speed_alpha1_gamma0.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\alpha_{OGD_V}\in[10\%,\;90\%]$}
        \label{fig:Hybrid_OGD_V_Speed_alpha1_gamma0}
    \end{subfigure}
    
    \caption{\texttt{OGD}$_V$ + $A_2$, \textbf{Fixed-Point Residues} and \textbf{$\bm{\epsilon}$-Nash Proximity} $(\gamma=0)$}
    \label{fig:OGD_V_Nash_Proximity_FixPoint}
\end{minipage}
\end{figure*}



%%%


In the final experiment, we assess convergence speed using both the $\epsilon$-Nash proximity and the fixed-point residual, reporting values at the final iteration $T$.  
Figure~\ref{fig:Hybrid_epsilon_error_alpha1_gamma0} shows that the $\epsilon$-Nash proximity increases with $\alpha_{\texttt{BR}}$, indicating that the system moves farther from the Nash equilibrium as \texttt{BR} becomes dominant. This behavior is consistent with earlier results, as non-\texttt{BR} users are increasingly penalized.  
The same trend persists under heterogeneous populations (Appendix Figs.~\ref{fig:Hybrid_epsilon_error_alpha1_gamma5}--\ref{fig:Hybrid_epsilon_error_alpha1_gamma10}).  
Figure~\ref{fig:Hybrid_Speed_alpha1_gamma0} further shows that all hybrid combinations (\texttt{BR}+\texttt{OGD}, \texttt{BR}+\texttt{DAQ}, \texttt{BR}+\texttt{RRM}) eventually stabilize and converge to a similar region, though not necessarily exactly at the Nash point.  
At the extreme $\alpha_{\texttt{BR}}=90\%$ (Figs.~\ref{fig:9_SBRD_1_epsilon_error_alpha1_gamma0}--\ref{fig:9_SBRD_1_Fix_Point_Err_alpha1_gamma0}), strong oscillations reappear and convergence may fail.

A different behavior arises when two no-regret algorithms interact.  
Figures~\ref{fig:OGD_V_Nash_Proximity_FixPoint} show the dynamics of \texttt{OGD}$_V$ mixed with either \texttt{DAQ}$_F$ or \texttt{RRM}$_V$.  
In these cases, both metrics exhibit a clear symmetry around the balanced configuration $\alpha_{\texttt{OGD}_V}=50\%$.  
Stability improves as $\alpha_{\texttt{OGD}_V}$ increases up to $50\%$, while beyond this point the dynamics degrade symmetrically, corresponding to the opposite imbalance in favor of the competing algorithm.  
This contrasts with \texttt{BR}+$\texttt{OGD}_V$ mixtures, where increasing dominance of $\texttt{OGD}_V$ consistently improves convergence.

%This contrasts with the \texttt{BR}+$A_2$ mixtures, where increasing the dominance of \texttt{BR} generally amplifies divergence from the Nash equilibrium.



\medskip


\noindent\textbf{Summary of findings.}  
(i) In the homogeneous dynamics, both homogeneous and heterogeneous populations maintain near-optimal efficiency across all learning rules.  

(ii) In hybrid populations, algorithmic imbalance strongly affects payoffs and efficiency; some stable hybrid outcomes yield utilities exceeding the Nash benchmark, confirming that the Kelly-game NE is not Pareto-optimal.   

(iii) Mixing \texttt{BR} with a no-regret method yields more stable and efficient outcomes than mixing two no-regret methods under strong imbalance.

\begin{comment}
\subsubsection{\textbf{Impact of utility curvature on efficiency}}
For linear valuation, with utilities $\varphi_i(\bm{z})\equiv a_ix_i(\bm{z})+ d_i - z_i$, the game admits a well-defined Nash equilibrium and convergence under no-regret learning~\cite{even2009convergence,Mertikoupoulous_ComNet_17}. However, the associated welfare ($\mathrm{SW}(\bm{z})=\sum_{i=1}^n a_ix_i(\bm{z}) + d_i$) maximization problem is affine and may admit multiple optimal solutions, for instance in the case of homogeneous agents. In heterogeneous settings, the linear welfare optimum typically corresponds to a greedy allocation that concentrates the resource on agents with the largest valuations ($\arg\max_i a_i$). In contrast, logarithmic valuations, with correspond utilities~\eqref{e:log_utility}, introduce curvature, yielding a unique welfare-optimal (not greedy) allocation while preserving equilibrium existence and learnability. We compare these two cases to quantify how utility curvature impacts relative efficiency loss.

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\linewidth]{img/Log_vs_Linear/bar_gamma_curvature_n_2.pdf}
        \caption{$n=2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\linewidth]{img/Log_vs_Linear/bar_gamma_curvature_n_4.pdf}
        \caption{$n=4$}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\linewidth]{img/Log_vs_Linear/bar_gamma_curvature_n_10.pdf}
        \caption{$n=10$}
    \end{subfigure}

\caption{Relative efficiency loss $\rho(\bm z(T))$ versus agent heterogeneity $\gamma$ for linear and logarithmic utilities, shown for different population sizes $n\in\{2,4,10\}$. Bars report final efficiency loss under identical learning dynamics.}

    \label{fig:linear_vs_log}
\end{figure}
Figure~\ref{fig:linear_vs_log} shows that logarithmic valuations consistently yield lower efficiency loss than linear valuations across all levels of heterogeneity, indicating improved robustness of social welfare outcomes. Figure~\ref{fig:linear_vs_log} further shows that logarithmic valuations benefit not only from heterogeneity robustness but also from scalability: the relative efficiency loss decreases as the number of agents $n$ increases ($\gamma$ fixed), even in heterogeneous populations. In contrast, for linear, efficiency loss decreases with $n$ only in the homogeneous case ($\gamma=0$), while remaining high under heterogeneity. This highlights that curvature improves both robustness to heterogeneity and efficiency scaling with the population size.
\end{comment}


%Table~\ref{tab:algorithms} summarizes Fig.~\ref{} simulations setting, e.g: in the column of Simulation $2$ $\text{Sim}_2$  means that $k$ player(s) use BRD and $n-k$ DAQ. The objectives of these simulations is 

 
\subsection{Figures omitted}
\label{app:Fifures}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t]
\centering

% ================= LEFT MINIPAGE ==================
\begin{minipage}{0.48\textwidth}
    \centering

    % Legend
    \includegraphics[width=\linewidth]{img/Non_Hybrid/Legend.pdf}

    % Subfigures
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{img/Non_Hybrid/Epsilon_Error/epsilon_error_alpha1_gamma0.0_n_10_plot.pdf}
        \caption{$\gamma=0$}
        \label{fig:epsilon_error_alpha1_gamma0}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{img/Non_Hybrid/Epsilon_Error/epsilon_error_alpha1_gamma5.0_n_10_plot.pdf}
        \caption{$\gamma=5$}
        \label{fig:epsilon_error_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{img/Non_Hybrid/Epsilon_Error/epsilon_error_alpha1_gamma10.0_n_10_plot.pdf}
        \caption{$\gamma=10$}
        \label{fig:epsilon_error_alpha1_gamma10}
    \end{subfigure}

    % Caption for this metric only
    \caption{Homogeneous dynamics: \textbf{$\epsilon$-Nash proximity} under different values of $\gamma$.}
    \label{fig:epsilon_summary}
\end{minipage}
\begin{minipage}{0.48\textwidth}

    \centering

    % Legend
    \includegraphics[width=\linewidth]{img/Non_Hybrid/Legend.pdf}

    % Subfigures
    \begin{subfigure}[b]{0.32\linewidth}
      \makebox[0pt][l]{\raisebox{.0cm}{\hspace*{0.7cm}\scriptsize$\rho(\mathbf{z}(T))=0.004\%$}}
        \includegraphics[width=\linewidth]{img/Non_Hybrid/Loss/All_Relative_Efficienty_Loss_alpha1_gamma0.0_n_10_plot.pdf}
        \caption{$\gamma=0$}
        \label{fig:SBRD_REL_alpha1_gamma0_n_10}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \makebox[0pt][l]{\raisebox{.0cm}{\hspace*{.7cm}\scriptsize$\rho(\mathbf{z}(T))=0.012\%$}}
        \includegraphics[width=\linewidth]{img/Non_Hybrid/Loss/All_Relative_Efficienty_Loss_alpha1_gamma5.0_n_10_plot.pdf}
        \caption{$\gamma=5$}
        \label{fig:SBRD_REL_alpha1_gamma5_n_10}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
        \makebox[0pt][l]{\raisebox{.0cm}{\hspace*{.7cm}\scriptsize$\rho(\mathbf{z}(T))=0.056\%$}}
        \includegraphics[width=\linewidth]{img/Non_Hybrid/Loss/All_Relative_Efficienty_Loss_alpha1_gamma10.0_n_10_plot.pdf}
        \caption{$\gamma=10$}
        \label{fig:SBRD_REL_alpha1_gamma10_n_10}
    \end{subfigure}

    % Caption for this metric only
    \caption{homogeneous dynamics: \textbf{Relative Efficiency Loss} under different values of $\gamma$.}
    \label{fig:REL_summary}

\end{minipage}



\end{figure*}

\begin{figure*}[!t]
\centering
    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=0.3\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]
\begin{minipage}{0.48\textwidth}
    \centering

    %--- Ligne de sous-figures (4 colonnes) ---
  \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Loss/Relative_Efficienty_Loss_alpha1_gamma5.0_player_plot.pdf}
        \end{overpic}
        \caption{$\gamma=5$}
        \label{fig:Hybrid_Relative_Efficienty_Loss_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Loss/Relative_Efficienty_Loss_alpha1_gamma10.0_player_plot.pdf}

        \end{overpic}
        \caption{$\gamma=10$}
        \label{fig:Hybrid_Relative_Efficienty_Loss_alpha1_gamma10}
    \end{subfigure}
    \caption{Hybrid setting: \texttt{SBRD} + $A_2$, \textbf{Relative Efficienty Loss} $(\gamma,\alpha_{SBRD})$}
    \label{fig_app:Hybrid_Relative_Efficienty_Loss}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering

    %--- Légende globale sur toute la largeur ---
    %\includegraphics[width=\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]


    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Loss/9_SBRD_1_Relative_Efficienty_Loss_alpha1_gamma5.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\gamma=5$}
        \label{fig:9_SBRD_1_Relative_Efficienty_Loss_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Loss/9_SBRD_1_Relative_Efficienty_Loss_alpha1_gamma10.0_n_10_plot.pdf}

        \end{overpic}
        \caption{$\gamma=10$}
        \label{fig:9_SBRD_1_Relative_Efficienty_Loss_alpha1_gamma10}
    \end{subfigure}
    \caption{Hybrid setting: \texttt{SBRD} + $A_2$, \textbf{Relative Efficienty Loss} $(\gamma,\alpha_{SBRD}=90\%)$}
    \label{fig_app:9_SBRD_1_Relative_Efficienty_Loss}
\end{minipage}
\end{figure*}


\begin{figure*}[!t]
\centering
    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=0.3\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]
\begin{minipage}{0.48\textwidth}
    \centering



    %--- Ligne de sous-figures (4 colonnes) ---

    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/epsilon_error_alpha1_gamma5.0_player_plot.pdf}
        \end{overpic}
        \caption{$\gamma=5$}
        \label{fig:Hybrid_epsilon_error_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/epsilon_error_alpha1_gamma10.0_player_plot.pdf}
        \end{overpic}
        \caption{$\gamma=10$}
        \label{fig:Hybrid_epsilon_error_alpha1_gamma10}
    \end{subfigure}
    \caption{Hybrid setting: \texttt{SBRD} + $A_2$, \textbf{$\bm{\epsilon}$-Nash Proximity} $(\gamma,\alpha_{SBRD})$}
    \label{fig_app:Hybrid_epsilon_error}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering

    %--- Ligne de sous-figures (4 colonnes) ---
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/9_SBRD_1_epsilon_error_alpha1_gamma5.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\gamma=5$}
        \label{fig:9_SBRD_1_epsilon_error_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/9_SBRD_1_epsilon_error_alpha1_gamma10.0_n_10_plot.pdf}

        \end{overpic}
        \caption{$\gamma=10$}
        \label{fig:9_SBRD_1_epsilon_error_alpha1_gamma10}
    \end{subfigure}
    \caption{Hybrid setting: \texttt{SBRD} + $A_2$, \textbf{$\bm{\epsilon}$-Nash Proximity} $(\gamma,\alpha_{SBRD}=90\%)$}
    \label{fig_app:9_SBRD_1_epsilon_error}
\end{minipage}
\end{figure*}





\begin{figure*}[!t]
    %--- Légende globale sur toute la largeur ---
    \centering
    \includegraphics[width=0.3\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]
\begin{minipage}{0.48\textwidth}
    \centering

    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/Speed_alpha1_gamma5.0_player_plot.pdf}
        \end{overpic}
        \caption{$\gamma=5$}
        \label{fig:Hybrid_Speed_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/Speed_alpha1_gamma10.0_player_plot.pdf}
        \end{overpic}
        \caption{$\gamma=10$}
        \label{fig:Hybrid_Speed_alpha1_gamma10}
    \end{subfigure}
    \caption{Hybrid setting: \texttt{SBRD} + $A_2$, \textbf{Fixed-Point Residues} $(\gamma,\alpha_{SBRD})$}
    \label{fig_app:Hybrid_Speed}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering

    %--- Légende globale sur toute la largeur ---
   % \includegraphics[width=\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/9_SBRD_1_Speed_alpha1_gamma5.0_n_10_plot.pdf}
        % ---- Rectangle for zoom region ----
        % (x,y) = bottom-left corner of rectangle in percent coordinates of the image
        % (width,height) also in percent
        \put(28,10){\color{black}\linethickness{0.7pt}\framebox(65,10){}}
    
        % ---- Insert zoomed image ----
        \put(42.8,30.1){
            \includegraphics[width=0.45\textwidth]{img/Hybrid/Fix_Point_Err/Zoom_9_SBRD_1_Speed_alpha1_gamma5.0_n_10_plot.pdf}
        }
    
        % ---- Arrow connecting region to zoom ----
        \linethickness{1pt}
        \put(50,35){\vector(-1,-1){15}} % Adjust arrow slope and length if needed 
        \end{overpic}
        \caption{$\gamma=5$}
        \label{fig:9_SBRD_1_Fix_Point_Err_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/9_SBRD_1_Speed_alpha1_gamma0.0_n_10_plot.pdf}
        % ---- Rectangle for zoom region ----
        % (x,y) = bottom-left corner of rectangle in percent coordinates of the image
        % (width,height) also in percent
        \put(35,10){\color{black}\linethickness{0.7pt}\framebox(60,10){}}
    
        % ---- Insert zoomed image ----
        \put(42.8,30.1){
            \includegraphics[width=0.45\textwidth]{img/Hybrid/Fix_Point_Err/Zoom_9_SBRD_1_Speed_alpha1_gamma10.0_n_10_plot.pdf}
        }
    
        % ---- Arrow connecting region to zoom ----
        \linethickness{1pt}
        \put(50,35){\vector(-1,-1){15}} % Adjust arrow slope and length if needed 
        \end{overpic}
        \caption{$\gamma=10$}
        \label{fig:9_SBRD_1_Fix_Point_Err_alpha1_gamma10}
    \end{subfigure}
    \caption{Hybrid setting: \texttt{SBRD} + $A_2$, \textbf{Fixed-Point Residues} $(\gamma,\alpha_{SBRD}=90\%)$}
    \label{fig_app:9_SBRD_1_Nash_Proximity}
\end{minipage}
\end{figure*}




\begin{figure}[!t]
    \centering

    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=0.3\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]

    %--- Ligne de sous-figures (4 colonnes) ---

    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/Hybrid_OGD_V_epsilon_error_alpha1_gamma5.0_n_10_plot.pdf}
        % ---- Rectangle for zoom region ----
        % (x,y) = bottom-left corner of rectangle in percent coordinates of the image
        % (width,height) also in percent
        \put(27,10){\color{black}\linethickness{0.7pt}\framebox(60,10){}}
    
        % ---- Insert zoomed image ----
        \put(35.8,25.1){
            \includegraphics[width=0.45\textwidth]{img/Hybrid/Epsilon_Error/Zoom_Hybrid_OGD_V_epsilon_error_alpha1_gamma5.0_n_10_plot.pdf}
        }
    
        % ---- Arrow connecting region to zoom ----
        \linethickness{1pt}
        \put(42,35){\vector(-1,-1){15}} % Adjust arrow slope and length if needed
        \end{overpic}
        \caption{$\gamma=5$}
        \label{fig:Hybrid_OGD_V_epsilon_error_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Epsilon_Error/Hybrid_OGD_V_epsilon_error_alpha1_gamma10.0_n_10_plot.pdf}
        % ---- Rectangle for zoom region ----
        % (x,y) = bottom-left corner of rectangle in percent coordinates of the image
        % (width,height) also in percent
        \put(27,10){\color{black}\linethickness{0.7pt}\framebox(60,10){}}
    
        % ---- Insert zoomed image ----
        \put(35.8,25.1){
            \includegraphics[width=0.45\textwidth]{img/Hybrid/Epsilon_Error/Zoom_Hybrid_OGD_V_epsilon_error_alpha1_gamma10.0_n_10_plot.pdf}
        }
    
        % ---- Arrow connecting region to zoom ----
        \linethickness{1pt}
        \put(42,35){\vector(-1,-1){15}} % Adjust arrow slope and length if needed
        \end{overpic}
        \caption{$\gamma=10$}
        \label{fig:Hybrid_OGD_V_epsilon_error_alpha1_gamma10}
    \end{subfigure}
    \caption{Hybrid setting: \texttt{OGD$_V$} + $A_2$, \textbf{$\bm{\epsilon}$-Nash Proximity} $(\gamma,\alpha_{OGD_V})$}
    \label{fig_app:Hybrid_OGD_V_epsilon_error}
\end{figure}

\begin{figure}[!t]
    \centering

    %--- Légende globale sur toute la largeur ---
    \includegraphics[width=0.3\textwidth]{img/Hybrid/legend.pdf}\\[0.5ex]

    %--- Ligne de sous-figures (4 colonnes) ---

    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/Hybrid_OGD_V_Speed_alpha1_gamma5.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\gamma=5$}
        \label{fig:Hybrid_OGD_V_Speed_alpha1_gamma5}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \begin{overpic}[width=\linewidth]
            {img/Hybrid/Fix_Point_Err/Hybrid_OGD_V_Speed_alpha1_gamma10.0_n_10_plot.pdf}
        \end{overpic}
        \caption{$\gamma=10$}
        \label{fig:Hybrid_OGD_V_Speed_alpha1_gamma10}
    \end{subfigure}
    \caption{Hybrid setting: \texttt{OGD$_V$} + $A_2$, \textbf{Fixed-Point Residues} $(\gamma,\alpha_{OGD_V})$}
    \label{fig_app:Hybrid_OGD_V_Speed}
\end{figure}











